NextStep-1: Toward Autoregressive Image Generation with Continuous Tokens at Scale

Prevailing autoregressive (AR) models for text-to-image generation either rely on heavy, computationally-intensive diffusion models to process continuous image tokens, or employ vector quantization (VQ) to obtain discrete tokens with quantization loss. In this paper, we push the autoregressive paradigm forward with NextStep-1, a 14B autoregressive model paired with a 157M flow matching head, training on discrete text tokens and continuous image tokens with next-token prediction objectives. NextStep-1 achieves state-of-the-art performance for autoregressive models in text-to-image generation tasks, exhibiting strong capabilities in high-fidelity image synthesis. Furthermore, our method shows strong performance in image editing, highlighting the power and versatility of our unified approach. To facilitate open research, we will release our code and models to the community.

==> chapters/conclusions.tex <==
\section{Limitations and Future Work}



==> chapters/data.tex <==
\section{Data \label{Section Data}}
NextStep-Gen is trained on a diverse set of datasets spanning multiple modalities, including languages, images, and videos.

\begin{figure*}[!htbp]
  \centering
  \centering
    \includegraphics[width=\linewidth]{figs/t2i_data.pdf}
    \caption{\textbf{Text-to-Image.}}
    \vspace{-0.5cm}
  \label{t2i.png}
\end{figure*}

\begin{figure*}[!htbp]
  \centering
  \centering
    \includegraphics[width=0.95\linewidth]{figs/edit_data.pdf}
    % \includegraphics[height=\textheight]{figs/edit_data.pdf}
    \caption{\textbf{Image-to-Image.}}
    \vspace{-0.5cm}
  \label{image_editing_data.png}
\end{figure*}

\begin{figure*}[!htbp]
  \centering
  \centering
    \includegraphics[width=\linewidth]{figs/interleaved_data.pdf}
    \caption{\textbf{interleave.}}
    \vspace{-0.5cm}
  \label{interleave.png}
\end{figure*}



\subsection{Single-Modality Data.}
\paragraph{Text-Only.} We use the part of language data as in dolma~\citep{dolma} and Step1o, which covers multilingual and rich text tasks to maintain the general language modeling capabilities.


\paragraph{Image-Only.} We extract multiple frames from the reality videos used in StepVideo~\citep{Step-Video-T2V}, and filter videos that contain subtitles and have low aesthetics.

\subsection{Text-to-Image Pairs.} 


\subsection{Image-to-Image Pairs.} We cruted a 

\subsection{Interleaved Data.}


\begin{table}[!h]
\centering
\begin{tabular}{ccc}
\toprule
Data Source                 & \# Data (M) & Sub-Task \\
\midrule
Image-Only             &             &               \\
Text-Only             &             &               \\
Text-to-Image Pair             &             &               \\
Image-to-Image Pair          &             &              \\
Interleaved Data &             &              \\
\bottomrule
\end{tabular}
\caption{\textbf{Data Type.}  \label{table:Pretrain-Data}}
\end{table}

\section{Training}

As shown in \Cref{table:Training recipe}, the training of NextStep-Gen is divided into five stages\footnote{In all stages, our VAE is frozen and other parameters are trained.}--- Pre-Training stage to acquire rich world knowledge, Continue-Training stage to learn natural image resolution, Cool-Down stage for improving image quality, Supervised Fine-Tuning stage for instruction following, and Reinforcement Learning stage for aligning human feedback:

\begin{itemize}
    \item \textbf{Stage1: General Pre-Training (PT)}. In this stage, we train all model parameters using a large and diverse training corpus of 2.8B samples, comprising text-only, image-only, text–to-image pairs, image-to-image pairs, and interleaved data. To expand the knowledge scope, text-image pairs from image understanding of Step 1o are also introduced and reordered. To learn more samples in the same training steps, we filter the images that are below $256 \times 256$ and resize all other images to a fixed resolution of $256 \times 256$. 
    
    \item \textbf{Stage2: Continue-Training (CT).} During this stage, we train the model with a dynamic resolution strategy and filter the images that are below $256 \times 256$ and larger than $2048 \times 2048$. Specifically, we have $4 \times 17$ buckets with different aspect ratios, and the images are assigned to the nearest buckets for training. Due to our model applying per-token image generation, we do not change any strategy for high resolution.  Besides, we increase the sampling ratio of OCR, editing, and interleaved video data, as these data need high image resolution.
    
    \item \textbf{Stage3: Cool-Down (CD).} Compared with PT and CT, we only use high-quality data in the cool-down stage.
    
    \item \textbf{Stage4: Supervised Fine-Tuning (SFT).} In the SFT stage, we construct instruction‑tuning data.  

    \item \textbf{Stage5: Reinforcement Learning (RL).} In the last stage, we enhance the OCR, xxx with multi-reward models.
\end{itemize}

In the training, NextStep-Gen treats texts and images as sequential tokens with a unified modeling strategy.

\input{tabs/training_recipe}

==> tabs/imgedit.tex <==
\begin{table}[!ht]
\centering
\scriptsize
\caption{\small \textbf{Comparison on ImgEdit-Bench.}}
% \vspace{0.2cm}
\resizebox{\columnwidth}{!}{
\begin{tabular}{lcccccccccc}
\toprule
\textbf{Model} & \textbf{Add} & \textbf{Adjust} & \textbf{Extract} & \textbf{Replace} & \textbf{Remove} & \textbf{Background} & \textbf{Style} & \textbf{Hybrid} & \textbf{Action} & \textbf{Overall} \\
\midrule
\textbf{\textit{Proprietary}} \\
\midrule
GPT-4o~\citep{openai2024gpt4o_image} & 4.61 & 4.33 & 2.90 & 4.35 & 3.66 & 4.57 & 4.93 & 3.96 & 4.89 & 4.20 \\
\midrule
\textbf{\textit{Open-source}} \\
\midrule
Instruct-Pix2Pix~\citep{Brooks2022InstructPix2PixLT} & 2.45 & 1.83 & 1.44 & 2.01 & 1.50 & 1.44 & 3.55 & 1.20 & 1.46 & 1.88 \\
MagicBrush~\citep{zhang2023magicbrush} & 2.84 & 1.58 & 1.51 & 1.97 & 1.58 & 1.75 & 2.38 & 1.62 & 1.22 & 1.90 \\
AnyEdit~\citep{yu2024anyedit} & 3.18 & 2.95 & 1.88 & 2.47 & 2.23 & 2.24 & 2.85 & 1.56 & 2.65 & 2.45 \\
UltraEdit~\citep{zhao2024ultraedit} & 3.44 & 2.81 & 2.13 & 2.96 & 1.45 & 2.83 & 3.76 & 1.91 & 2.98 & 2.70 \\
OmniGen~\citep{xiao2024omnigen} & 3.47 & 3.04 & 1.71 & 2.94 & 2.43 & 3.21 & 4.19 & 2.24 & 3.38 & 2.96 \\
OmniGen2~\citep{wu2025omnigen2} & 3.57 & 3.06 & 1.77 & 3.74 & 3.20 & 3.57 & 4.81 & 2.52 & 4.68 & 3.44 \\
Step1X-Edit v1.0~\citep{liu2025step1xeditpracticalframeworkgeneral} & 3.88 & 3.14 & 1.76 & 3.40 & 2.41 & 3.16 & 4.63 & 2.64 & 2.52 & 3.06 \\
ICEdit~\citep{zhang2025ICEdit} & 3.58 & 3.39 & 1.73 & 3.15 & 2.93 & 3.08 & 3.84 & 2.04 & 3.68 & 3.05 \\
BAGEL~\citep{deng2025emerging} & 3.56 & 3.31 & 1.70 & 3.30 & 2.62 & 3.24 & 4.49 & 2.38 & 4.17 & 3.20 \\
Flux.1-Kontext-dev~\citep{labs2025flux1kontextflowmatching} & 3.76 & 3.45 & 2.15 & 3.98 & 2.94 & 3.78 & 4.38 & 2.96 & 4.26 & 3.52 \\
GPT-Image-Edit~\citep{wang2025gpt-edit-1_5M} & 4.07 & 3.79 & 2.04 & 4.13 & 3.89 & 3.90 & 4.84 & 3.04 & 4.52 & 3.80 \\
\rowcolor{myblue}
\Ours \\
\bottomrule
\end{tabular}
}
\label{tab:imgedit}
\end{table}

==> tabs/inference_time.tex <==
\begin{table}[ht]
\centering
\caption{\small Title}
\begin{tabular}{ccccccc}
\toprule
\textbf{H100 TFLOPS} & \textbf{Memory Bandwidth} & \textbf{LM Decoder} & \textbf{LM Head} & \textbf{Flow Matching Head} & \textbf{Accumulated Time} &
\textbf{Accumulated Time w/o FM Head} \\
\midrule
% 16,384 & 3.2 TB/s & 10.5s & 2.1s & 1.5s & 14.1s & 12.6s \\
... & ... & ... & ... & ... & ... & ... \\
... & ... & ... & ... & ... & ... & ... \\
\bottomrule
\end{tabular}
\label{tab:inference_time}
\end{table}
